A Generalization of Wirtinger Flow for Exact Interferometric Inversion

Interferometric inversion involves recovery of a signal from cross-correlations of its linear transformations. A close relative of interferometric inversion is the generalized phase retrieval problem, which consists of recovering a signal from the auto-correlations of its linear transformations. Recently, significant advancements have been made in phase retrieval methods despite the ill-posed, and non-convex nature of the problem. One such method is Wirtinger Flow (WF), a non-convex optimization framework that provides high probability guarantees of exact recovery under certain measurement models, such as coded diffraction patterns, and Gaussian sampling vectors. In this paper, we develop a generalization of WF for interferometric inversion, which we refer to as Generalized Wirtinger Flow (GWF). GWF theory extends the probabilistic exact recovery results of WF to arbitrary measurement models characterized in the equivalent lifted problem, hence covers a larger class of measurement models. Our framework unifies the theory of low rank matrix recovery (LRMR) and the non-convex optimization approach of WF, thereby establishes theoretical advantages of the non-convex approach over LRMR. We identify a new sufficient condition on the lifted forward model that directly implies exact recovery conditions of standard WF. This condition is less stringent than those of LRMR, which is the state of the art approach for exact interferometric inversion. We establish our sufficient condition for the cross-correlations of linear measurements collected by complex Gaussian sampling vectors, and show that the exact recovery conditions of standard WF imply our sufficient condition. As a result, the regularity condition of WF becomes redundant in solving the interferometric inversion problem. Finally, we demonstrate the effectiveness of GWF numerically in a deterministic multi-static radar imaging scenario.

==> Proof_Of_Lemma6.tex <==
From the adjoint property of the inner product we have
$$ \| \mathcal{F} ( \brho \brho^H - \brho_t \brho_t^H ) \|^2 = \langle \brho \brho^H - \brho_t \brho_t^H , \mathcal{F}^H \mathcal{F} ( \brho \brho^H - \brho_t \brho_t^H ) \rangle_F.$$ Splitting the linear operator $\mathcal{F}^H \mathcal{F}$ over the rank-1 inputs, we can use the perturbation model from Lemma  \ref{cor:Corr1} such that
\begin{eqnarray}
& = & \langle \brho \brho^H - \brho_t \brho_t^H , \mathcal{F}^H \mathcal{F} (\brho \brho^H ) \rangle_F -  \langle \brho \brho^H - \brho_t \brho_t^H , \mathcal{F}^H \mathcal{F} (\brho_t \brho_t^H ) \rangle_F \nonumber \\
& = & \| \brho \brho^H - \brho_t \brho_t^H \|_F^2 + \langle \brho \brho^H - \brho_t \brho_t^H, \bdelta(\brho \brho^H) - \bdelta( \brho_t \brho_t^H) \rangle_F. \label{eq:App6_eq1}
\end{eqnarray}
%& = & \langle \brho \brho^H - \brho_t \brho_t^H ,  \brho \brho^H + \bdelta(\brho \brho^H) \rangle_F -  \langle \brho \brho^H - \brho_t \brho_t^H , \brho_t \brho_t^H + \bdelta (\brho_t \brho_t^H ) \rangle_F \nonumber \\

Using the representation of $\tilde{\mathbf{e}} = \brho \brho^H - \brho_t \brho_t^H$ in \eqref{eq:lifted_Error_fin_app5}, and the linearity of $\bdelta$ we get %and extending the domain of $\bdelta$ on the set of rank-1 matrices, from the linearity of $\bdelta$ we have
\begin{equation}\label{eq:App6_eq2_v1}
\bdelta(\brho \brho^H) - \bdelta(\brho_t \brho_t^H) = \bdelta(\brho_e \brho_e^H) + \bdelta(\brho_e \hat{\brho}_t^H + \hat{\brho}_t \brho_e^H). 
\end{equation}
Notably, the domain of $\bdelta$ is by definition the set of rank-1, PSD matrices. 
Having $\brho_e \hat{\brho}_t^H + \hat{\brho}_t \brho_e^H$, a symmetric matrix of at most rank-2 in the argument of $\bdelta$ on the right-hand-side, we can represent \eqref{eq:App6_eq2_v1} by an eigenvalue decomposition and use the linearity of $\bdelta$ to obtain
\begin{equation}\label{eq:App6_eq2}
\bdelta(\brho \brho^H) - \bdelta(\brho_t \brho_t^H)  = \bdelta(\brho_e \brho_e^H) + \lambda_1 \bdelta(\v_1 \v_1^H) + \lambda_2 \bdelta(\v_2 \v_2^H),
\end{equation}
where $\brho_e \hat{\brho}_t^H + \hat{\brho}_t \brho_e^H = \sum_{i =1}^2 \lambda_i \v_i \v_i^H$. 

Plugging \eqref{eq:App6_eq2} into \eqref{eq:App6_eq1}, and applying Cauchy-Schwartz and triangle inequalities on absolute value of the Frobenius inner product term, we have
%\begin{equation}
%\| \mathcal{F} ( \brho \brho^H - \brho_t \brho_t^H ) \|^2 = \| \brho \brho^H - \brho_t \brho_t^H \|_F^2 + \langle \brho \brho^H - \brho_t \brho_t^H, \bdelta(\brho_e \brho_e^H) + \bdelta( \brho_e \hat{\brho}_t^H )  + \bdelta( \hat{\brho}_t \brho_e^H) \rangle_F
%\end{equation}
\begin{equation}\label{eq:App6_eq3}
\begin{split}
& | \langle \brho \brho^H - \brho_t \brho_t^H, \bdelta(\brho \brho^H) - \bdelta( \brho_t \brho_t^H) \rangle_F |  \leq  \cdots \\
 & \cdots \| \brho \brho^H - \brho_t \brho_t^H \|_F \left(\| \bdelta(\brho_e \brho_e^H)\|_F + |\lambda_1| \| \bdelta( \v_1 \v_1^H ) \|_F  + |\lambda_2| \| \bdelta( \v_2 \v_2^H)  \|_F \right).
\end{split}
\end{equation}
%$$
%\leq \| \brho \brho^H - \brho_t \brho_t^H \|_F \left(\| \bdelta(\brho_e \brho_e^H)\|_F +  \| \bdelta( \brho_e \hat{\brho}_t^H ) \|_F  + \| \bdelta( \hat{\brho}_t \brho_e^H)  \|_F \right).
%\end{equation}
Furthermore, from Lemma \ref{cor:Corr1}, for a RIP-1 property of $\mathcal{F}$ with RIC-$\delta_1$, for \eqref{eq:App6_eq3} we have
\begin{eqnarray}
& \leq &\delta_1 \| \brho \brho^H - \brho_t \brho_t^H \|_F \left(\| \brho_e \brho_e^H \|_F +  |\lambda_1| + |\lambda_2| \right) \nonumber \\
& \leq &  \delta_1  \| \brho \brho^H - \brho_t \brho_t^H \|_F \left(\| \brho_e \brho_e^H \|_F +  \|  \brho_e \hat{\brho}_t^H \|_* + \| \hat{\brho}_t \brho_e^H  \|_* \right), \label{eq:App6_eq4}
\end{eqnarray}
where we use the fact that $\| \v_1 \| = \| \v_2 \| = 1$, and $\| \brho_e \hat{\brho}_t^H   + \hat{\brho}_t \brho_e^H \|_* =  | \lambda_1 | + | \lambda_2 |$ by definition, from on which the triangle inequality follows.  
Invoking the rank-1 property on the terms inside the parenthesis in \eqref{eq:App6_eq4}, the Frobenius norm and the nuclear norms can be computed by the spectral norm, since $\| \cdot \| = \| \cdot \|_F = \| \cdot \|_*$ for a rank-1 argument. 
Then, having $ \| \brho_t \| = 1$, for the right-hand-side we obtain
\begin{eqnarray}
| \langle \brho \brho^H - \brho_t \brho_t^H, \bdelta(\brho \brho^H) - \bdelta( \brho_t \brho_t^H) \rangle_F | &\leq & \delta_1  \| \brho \brho^H - \brho_t \brho_t^H \|_F \left(2 \| \brho_t \| \| \brho_e \| + \| \brho_e \|^2 \right) \nonumber \\
& \leq & \delta_1 (2 + \epsilon)  \| \brho \brho^H - \brho_t \brho_t^H \|_F \ \text{dist}( \brho, \brho_t ). 
\end{eqnarray}
Using the bound 
\begin{equation}
\sqrt{(1-\epsilon)(2-\epsilon)} \text{dist}(\brho, \brho_t) \leq \| \brho \brho^H - \brho_t \brho_t^H \|_F,
\end{equation}
from Lemma \ref{lem:Lemma5}, we finally obtain the upper bound on the perturbation on $ \| \brho \brho^H - \brho_t \brho_t^H \|_F^2 $ as
\begin{equation}
| \langle \brho \brho^H - \brho_t \brho_t^H, \bdelta(\brho \brho^H) - \bdelta( \brho_t \brho_t^H) \rangle_F |  \leq \delta_1 \frac{2+\epsilon}{\sqrt{(1-\epsilon)(2-\epsilon)}} \| \brho \brho^H - \brho_t \brho_t^H \|_F^2.
\end{equation}
Hence, setting $\delta_2 = \delta_1 \frac{2+\epsilon}{\sqrt{(1-\epsilon)(2-\epsilon)}}$, we have the local RIP-2 condition satisfied with RIC-$\delta_2$. 


